Persistence and Synchronization: Friends or Foes?

Emerging non-volatile memory (NVM) technologies promise memory speed byte-addressable persistent storage with a load/store interface. However, programming applications to directly manipulate NVM data is complex and error-prone. Applications generally employ libraries that hide the low-level details of the hardware and provide a transactional programming model to achieve crash-consistency. Furthermore, applications continue to expect correctness during concurrent executions, achieved through the use of synchronization. To achieve this, applications seek well-known ACID guarantees. However, realizing this presents designers of transactional systems with a range of choices in how to combine several low-level techniques, given target hardware features and workload characteristics. In this paper, we provide a comprehensive evaluation of the impact of combining existing crash-consistency and synchronization methods for achieving performant and correct NVM transactional systems. We consider different hardware characteristics, in terms of support for hardware transactional memory (HTM) and the boundaries of the persistence domain (transient or persistent caches). By characterizing persistent transactional systems in terms of their properties, we make it possible to better understand the tradeoffs of different implementations and to arrive at better design choices for providing ACID guarantees. We use both real hardware with Intel Optane DC persistent memory and simulation to evaluate a persistent version of hardware transactional memory, a persistent version of software transactional memory, and undo/redo logging. Through our empirical study, we show two major factors that impact the cost of supporting persistence in transactional systems: the persistence domain (transient or persistent caches) and application characteristics, such as transaction size and parallelism.

==> Makefile <==
PAPER=paper
TARGET=paper

default: paper

pdf:
	GS_OPTIONS=-dPDFSETTINGS=/prepress rubber -e "bibtex.crossrefs 100" --pdf -Wrefs -Wmisc $(TARGET)

paper:
	pdflatex $(PAPER).tex </dev/null
	bibtex $(PAPER)
	pdflatex $(PAPER).tex </dev/null >/dev/null
	pdflatex $(PAPER).tex </dev/null >/dev/null
	pdflatex $(PAPER).tex </dev/null

clean:
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(TARGET).ps $(TARGET).pdf

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;


==> introduction.tex <==
% !TEX root = paper.tex

\section{Introduction}

Emerging Non-Volatile Memory (NVM) technologies, like Intel's 3D XPoint~\cite{3dxpoint},
offer orders of magnitude faster access to storage than traditional storage technologies.
One of their key appeals is that they allow applications to access storage directly using processor load and store instructions rather than relying on a software intermediary like the file system or a database~\cite{pelleychen14}.
However, ensuring that data stored in NVM is always in a safe and recoverable state (i.e., the data is \emph{crash-consistent}) is both hard and incurs performance overheads~\cite{bpfs,mnemosyne,nvheaps,pelleychen14}.
To ensure crash consistency, application developers have to carefully orchestrate the movement of data from the volatile to non-volatile components in the memory hierarchy subject to recoverability constraints.

To exacerbate the challenge of ensuring crash consistency, different systems provide different guarantees on when data may be considered persistent.
For example, Intel and Micron guarantee that data becomes persistent only when it reaches the memory controller of the NVM device, i.e., the persistent domain of the system includes the memory controller and the NVM devices~\cite{intel2016pcommit}.
We refer to such systems as having \emph{transient caches}.
However, HPE's NVM~\cite{hpnvdimm} guarantees that the entire cache hierarchy is persistent, i.e., the persistent domain of the system includes the entire memory hierarchy.
We refer to such systems as having \emph{persistent caches}.
Based on the persistent domain of the systems, developers have to tailor their applications to achieve crash consistency.
The diversity of NVM applications~\cite{whisper} further complicates achieving crash consistency.
Multi-threaded applications require developers to ensure correct synchronization on top of crash consistency.

One way to simplify the development of NVM applications is to use a single abstraction that provides guarantees on both crash consistency and correct synchronization. The transactional programming interface is particularly well suited for this approach as we have been using transactions to independently achieve crash consistency (e.g., database transactions) or proper synchronization (e.g., transactional memory systems). To this end, prior work has proposed numerous systems to simultaneously guarantee both these properties~\cite{mnemosyne,nvheaps,phtm,phytm,Wang:cal:2015,Joshi:isca:2018,Doshi:hpca:2016}.
While these systems provide transactions with the desirable ACID properties that permit their use for both \cc and \sync, they do so in a they do so in a myriad of ways, some implemented completely in software while some rely on hardware support, some use undo logging, while others use redo logging. So, developers are faced with a bewildering array of choices, with varied performance characteristics that change with applications and the system used. For a platform with given hardware features and consistency and synchronization requirements, is it possible to streamline the design space and quickly arrive at a correct and performant implementation of a transactional system?

\begin{comment}
One way to simplify the development of NVM applications is to use a single abstraction that provides guarantees on both crash consistency and correct synchronization.
To efficiently describe the properties of a system providing both \cc and correct \sync simultaneously for the same data, we coin the term \csty (\S\ref{pvs}).
The transactional programming interface is particularly well suited for this approach as we have been using transactions to independently achieve crash consistency (e.g., database transactions) or
proper synchronization (e.g., transactional memory systems).
To this end, prior work has proposed numerous systems to simultaneously guarantee both these properties~\cite{mnemosyne,nvheaps,phtm,phytm,Wang:cal:2015,Joshi:isca:2018,Doshi:hpca:2016}.
While these systems \ada{provide full ACID transactions and} guarantee \csty, they do so in a myriad of ways, some implemented completely in software while some rely on hardware support, some use undo logging, while others use redo logging.
So, developers are faced with a bewildering array of choices, with varied performance characteristics that change with applications and the system used.
\end{comment}

To efficiently describe the properties of a system providing both \cc and correct \sync simultaneously for the same data, we coin the term \csty (\S\ref{pvs}).
%In this work, 
\ada{We use \csty to characterize transaction systems with respect to their \cc requirements, impacted by the persistence domain, and \sync requirements, determined by the support for and use of concurrency. }
We perform a detailed study of 
%these 
systems \ada{with different characteristics} under various operating scenarios \ada{ and provide undertanding of the relationship of \csty and the best implementation of a transactional programming model for a given NVM system. }
% that developers can use before deciding on using a particular system.
%Specifically, we want to understand (1) what is the cost of ensuring \cc and \csty using a transactional programming model and (2) what is the best implementation of this model for various NVM systems. 
We implement and evaluate various methods for realizing the transactional programming model, 
\ada{by following closely the best designs presented in prior work}: hardware transactional memory (\htm) \cite{Joshi:isca:2018}, 
software transactional memory (\stm) \cite{mnemosyne}, and \undo/\redo logging with locks \cite{pmdk,mnemosyne}. 
Through emulation and simulation, we consider both transient and persistent caches and vary the latency characteristics of the NVM. 
Finally, we perform our characterization study on real hardware using the recently released Intel's DC Optane Persistent Memory~\cite{dcoptane}.

Our empirical study results in the following conclusions:\\
(1) In systems with transient caches, HTM benefits crash-consistency, despite its synchronization costs and required architectural changes. This is due to the high overheads caused by flush and fence instructions required by undo/redo logs elided by HTM. Moreover, the choice between undo and redo logs vastly depends on the application characteristics and the size of the read and write sets of the transactions. 
(2) In systems with persistent caches, the HTM’s benefit (without any architectural changes) for crash-consistency is reduced, as software logging mechanisms do not require expensive flush and fence instructions anymore. Moreover, undo logs are the best choice for ensuring crash-consistency when caches are persistent, since redo logs still suffer from read-indirection overheads. 
(3) We find that crash-consistent HTM design consistently outperforms other transactional implementations for transient caches as well as persistent caches. This shows that for transient caches extending HTM with crash-consistency is the most promising solution to provide crash-sync-safe transactions, 
%\ada{and discuss several optimizations over prior crash-consistent HTM designs -- but the benefits of the optimizations are not explicitly evaluated?}. -- It is hard and text consuming to sell our ccHTM superiority over others.
% lets not fight that battle (pradeep).
In addition, for persistent caches, current HTMs are already crash-sync-safe. 
(4) In multi-threaded applications, the persistence domain still plays a very important role. The overhead of crash-consistency is considerably lower when caches are persistent. In addition, HTM is crash-consistent out of the box, so no changes are necessary. 
(5) When using crash-consistent HTM to achieve crash-sync-safety, it comes almost for free. The overheads of crash-consistency are subsumed by synchronization overheads and, as applications scale, performance increases compared to single-thread execution. When the crash-consistent HTM does not achieve scalability due to aborts, the crash-consistent STM ensures this property. \ada{still needs some improvement for clarity. }



%(1) The persistence domain significantly impacts the performance and programmability of transactional libraries. The cost of \cc and \csty for persistent caches is \ic{XX\% and YY} lower than for transient caches\ic{, respectively}. This suggests that NVM manufacturers and datacenter admins should consider increasing the persistence domain to the cache hierarchy, whenever possible (e.g., by augmenting the system with a battery).
%(2) \cc has a non-trivial overhead for both persistent \ic{(XX\%)} and transient caches\ic{(XX\%)}. However, techniques for ensuring multi-threaded \sync, such as STM and HTM, can help alleviate some of this overhead by 
%enabling applications to scale. Therefore, \csty generally has lower overhead when employing multiple threads \ic{(XX for persistent caches and XX for transient caches)} than \cc. 
%(3) While the \htm and \stm techniques extended to guarantee \cc always outperform other methods for \csty for both persistent and transient caches, there is no clear winner between the two, as their behavior depends on the workload. 
%\ada{what's missing is that \htm and \stm need to be \cc too, with small hardware extensions. also better links the insights for Micro. }
%(4) For \cc, the overhead of the \stm is too high when the application does not scale to more threads. However, the \htm still outperforms \undo/\redo logs for transient caches because it reduces the number of fences required. For persistent caches, where fences are not required, the \undo log outperforms all other methods. 
%\jg{We need numbers here and need to update so that most are on real NVM not DRAM anymore except simulator}.

Overall, this paper makes the following contributions:
\begin{itemize}
	\item We introduce the notion of \csty and discuss \ada{how different system features (e.g., persistence domain, HTM support) and requirements (e.g., multi- vs.~single-threaded use) impacts the  implementation of this property. }
%how various system implementations can be used to achieve this property.
	\item We compare the performance of various systems guaranteeing \csty on systems with different persistent domains \ada{and different concurrency support and requirements}.
	\item We believe we are the first work to evaluate the performance of different \csty techniques on real 3D XPoint memory devices.
	\item We show that there is 
%no one best way to ensure \csty and in fact the best way changes with application and the persistent domain guarantees provided by the system. 
\ada{no one best way to ensure adequate transactional support in NVM-based systems, and in fact the best way changes with the \csty property of the system, impacted by its persistence domain, the presence and efficiency of hardware support for transactional concurrency control, and the application requirements. }
\end{itemize}


%The rest of the paper is organized as follows. First, we define \csty (\S\ref{pvs}) and discuss how to achieve it (\S\ref{sec:design}). Next, we explain our methodology (\S\ref{sec:methodology}), 
%and present an extensive evaluation of the 
%various implementations for \cc (\S\ref{sec:st}) and for \csty (\S\ref{sec:mt}).
%\ada{change to use top level label for Section 8}



%Emerging Non-Volatile Memory (NVM) technologies 
%(also known as persistent memories)
%are byte-addressable,
%offer a load-store interface to storage and approach DRAM speeds, which makes
%them orders of magnitude faster than traditional storage~\cite{3dxpoint}. 
%The traditional interface to storage, such as a file system's
%read/write system calls, becomes a performance bottleneck. 
%Future applications
%are expected to directly access storage via load/store instructions~\cite{pelleychen14}.
%
%Moreover, converting some of the transient in-memory application data to persistent data could result in shorter application downtime following a crash and faster recovery times. For example, an application that serves as a software cache to a backend storage server, traditionally would maintain the cached data as transient data in DRAM, and reconstruct the cache from the storage server on restart. Making the data persistent by storing it in NVM instead leads to faster warmup times, as the cache is already populated and does not need to start cold. 
%
%Although NVM is much faster than traditional storage, ensuring data persistence in NVM still suffers from 
%<<<<<<< HEAD
%However, ensuring data persistence in NVM suffers from 
%performance and programmability costs~\cite{bpfs,mnemosyne,nvheaps,pelleychen14}. 
%Developers need to ensure that the data stored in NVM is always in a recoverable
%state in the event of an unexpected system crash, i.e., that their applications are \emph{crash-consistent}. 

%Moreover, the huge diversity of NVM technologies already available on the market or soon to be available exacerbate the problem
%because they offer very different performance and consistency guarantees. 
%For example, HPE's NVM solution~\cite{hpnvdimm} offers similar performance 
%as DRAM and persistence throughout the memory hierarchy, including the 
%CPU caches (\emph{persistent caches}). 
%In contrast, Intel and Micron's proposed 3DXPoint technology~\cite{3dxpoint} has higher latency 
%and lower bandwidth than DRAM, while the persistence domain includes only the NVM and the memory 
%controller, but not the CPU caches (\emph{transient caches})~\cite{intel2016pcommit}.
%These characteristics have drastic impact on performance and programming models.
%\jg{Now that we have real NVM device, we may want to rephrase this paragraph}.

%Beyond the diversity of the NVM systems, the diversity of NVM workloads~\cite{whisper} adds even more complexity. Applications vary with the size of the crash-consistent regions, as well as the size of the read and write sets and the number of threads employed. In particular, multi-threaded applications need to ensure correct synchronization of shared data, in addition to crash-consistency. 
%=======
%However, ensuring data persistence in NVM suffers from 
%performance and programmability costs~\cite{bpfs,mnemosyne,nvheaps,pelleychen14}. 
%Developers need to ensure that the data stored in NVM is always in a recoverable
%state in the event of an unexpected system crash, i.e., that their applications are \emph{crash-consistent}. 

%Moreover, the huge diversity of NVM technologies already available on the market or soon to be available exacerbate the problem
%because they offer very different performance and consistency guarantees. 
%For example, HPE's NVM solution~\cite{hpnvdimm} offers similar performance 
%as DRAM and persistence throughout the memory hierarchy, including the 
%CPU caches (\emph{persistent caches}). 
%In contrast, Intel's newly released Intel Optane DC persistent memory, based on  
%3DXPoint technology~\cite{3dxpoint}, has higher latency 
%and lower bandwidth than DRAM, while the persistence domain includes only the NVM and the memory 
%controller, but not the CPU caches (\emph{transient caches})~\cite{intel2016pcommit}.
%These characteristics have drastic impact on performance and programming models.
%\jg{Now that we have real NVM device, we may want to rephrase this paragraph}.

%Beyond the diversity of the NVM systems, the diversity of NVM workloads~\cite{whisper} adds even more complexity. Applications vary with the size of the crash-consistent regions, as well as the size of the read and write sets and the number of threads employed. In particular, multi-threaded applications need to ensure correct synchronization of shared data, in addition to crash-consistency. 
%>>>>>>> 2fdbdaa39875df813652efb18eb78b6d0ceb6759
%
%One way to efficiently attain both crash consistency and synchronization is to use 
%an abstraction that can provide both properties simultaneously.
%Developers directly benefit from the simplicity of programming with transactions that achieve both 
%crash consistency and correct synchronization of shared data, relieving them from reasoning independently about consistency in the presence of failures and data visibility between threads. To efficiently describe the properties of a system that achieves both \cc and correct \sync simultaneously for the same data, we coin the term \cs (\S\ref{pvs}).

%In this paper, we explore the feasibility of converting transient data to persistent data stored on NVM.
%We consider transactional applications and convert the data accessed transactionally. 

%<<<<<<< HEAD
%In this paper, we want to understand (1) what is the cost of \cc and \cs using a transactional programming model and (2) what is the best implementation of this model for various NVM technologies with different characteristics and persistence domains. 
%We implement and evaluate various methods for realizing the transactional programming model: software transactional memory (\stm), hardware transactional memory (\htm), and \undo/\redo logging with locks. Through emulation and simulation, we consider both transient and persistent caches and we vary the latency characteristics of the NVM. We consider a variety of workloads with small and large transactions. 
%\jg{we are just going to evaluate 3Dxpoint (in my opinion), we need to change and say exactly we do that. We are relying to much on various NVM charateristics. Persistence domains still exists I assume.}
%=======
%In this paper, we want to understand (1) what is the cost of \cc and \cs using a transactional programming model and (2) what is the best implementation of this model for various NVM technologies with different characteristics and persistence domains. 
%We implement and evaluate various methods for realizing the transactional programming model: software transactional memory (\stm), hardware transactional memory (\htm), and \undo/\redo logging with locks. Through use of real hardware based on Intel's Optane PM and simulation, we consider both transient and persistent caches and we vary the latency characteristics of the NVM. We consider a variety of workloads with small and large transactions. 
%\jg{we are just going to evaluate 3Dxpoint (in my opinion), we need to change and say exactly we do that. We are relying to much on various NVM charateristics. Persistence domains still exists I assume.}
%>>>>>>> 2fdbdaa39875df813652efb18eb78b6d0ceb6759


%For persistent caches, \stm and \htm provide \cs. We use TinySTM~\cite{tinystm} as the STM and Intel Transactional Synchronization Extensions~\cite{inteltsx} (TSX) as the HTM. We use DRAM to emulate NVM with persistent caches. 
%
%For transient caches, we implement and evaluate a crash-consistent version of the \stm (\ccstm) and of the \htm (\cchtm). We combine emulation on real hardware and simulation using the SESC simulator~\cite{sesc} to analyze the performance implications of transient caches. 
%
%\undo/\redo logging provides only \cc. Where necessary to ensure \cs, we extend \undo/\redo with a global lock to provide correct \sync. 



%<<<<<<< HEAD
%Many works have explored the 
%use of transactions for both crash-consistency~\cite{atomic} and synchronization (transactional memory~\cite{Herlihy:1993}). 
%We build on this work 
%to make the following contributions: 
%=======
%Many works have explored the 
%use of transactions for both crash-consistency~\cite{atomic} and for synchronization (transactional memory~\cite{Herlihy:1993}). 
%We build on this work 
%to make the following contributions: 
%>>>>>>> 2fdbdaa39875df813652efb18eb78b6d0ceb6759
%
%(1) We introduce \cs and show that by scaling up, we can reduce the cost of \cc. 
%advocate that we should consider crash-consistency and synchronization together, since doing so has multiple benefits for applications. 
%We evaluate crash-consistency for single-threaded applications and crash-sync for multi-threaded applications. 
%
%(2) We are the first to evaluate \ccms across persistence domains. While prior work has evaluated crash-consistent versions of STM~\cite{mnemosyne,nvheaps} and HTM~\cite{phtm,phytm,Wang:cal:2015,Joshi:isca:2018,Doshi:hpca:2016} 
%for transient caches, we show the behavior of STM and HTM for persistent caches as well, and we analyze the differences in design, implementation and performance results caused by the persistence domain.  
%
%For persistent caches, \stm and \htm provide \cs. 
%We use TinySTM~\cite{tinystm} as the STM and Intel Transactional Synchronization Extensions~\cite{inteltsx} (TSX) as the HTM. 
%for persistent caches, because they already provide \cs. 
%<<<<<<< HEAD
%We use DRAM to emulate NVM with persistent caches. 
%=======
%We use DRAM to emulate NVM with persistent caches. \ada{Remote this sentence completely?}
%>>>>>>> 2fdbdaa39875df813652efb18eb78b6d0ceb6759
%
%(3) 
%For transient caches, we implement and evaluate a crash-consistent version of the \stm (\ccstm) and of the \htm (\cchtm). 
%We combine emulation on real hardware and simulation using the SESC simulator~\cite{sesc} to analyze the performance implications of transient caches. 
%
%We evaluate the HTM across both real hardware and architectural simulation, while prior work focused on one or the other. 
%An HTM on real hardware can only provide an approximation of a ccHTM, with only the fallback path being crash-consistent. Thus, we designed and 
%implemented an optimized version of a ccHTM in the SESC simulator~\cite{sesc}. Our ccHTM is similar to prior work in that we extend hardware transactions to log writes for crash-consistency, but differs in \emph{how we implement the log}. We use non-transactional non-temporal operations to write the log inside a hardware transaction, so that these writes are not part of the transaction's write set and do not cause conflicts or cache overflows.


%we analyze how to provide and what is its cost/performance implications. 

%In this paper, we explore the transactional programming model for both crash consistency and synchronization 
%simultaneously, by combining them in the same runtime. 
%Our goal is to understand 
%(1) the cost of supporting just crash consistency and the cost of supporting both crash consistency and synchronization;
%(2) if the transactional programming model can deliver good performance for single-threaded applications seeking 
%only crash consistency and for multi-threaded applications seeking both crash consistency and synchronization; 
%and (3) What is the best way (hardware, software, etc.) to implement a crash consistent transactional memory system
%for a range of application and NVM system characteristics?
%
%In particular, we consider both persistent and transient CPU caches, which 
%has profound implications on performance of a transactional system that supports both crash consistency and 
%synchronization.
%We implement and evaluate the transactional model using multiple mechanisms and we optimize each 
%one according to the different NVM technologies.


%
%Naturally, we first consider an implementation based on transactional memory. 
%When CPU caches are persistent, transactional memory provides both persistence and 
%synchronization without any changes.% to the implementation. 
%This is true for both hardware transactional memory (HTM) and software transactional memory (STM). 
%An HTM, such as 
%Intel's Transactional Synchronization Extensions (TSX), can provide persistence without any changes to the HTM implementation because 
%of its coherence protocol-based implementation. 
%Cache lines accessed within a transaction get buffered in the L1 cache and their eviction 
%causes the transaction to abort. Therefore, modified transactional cache lines cannot be evicted to NVM during the transaction and leave the 
%NVM in an inconsistent state. 
%If  a cache line gets 
%evicted for any reason, the transaction will be aborted and all the modified cache lines will be discarded. 
%An STM with deferred updates, such as TinySTM~\cite{tinystm}, stores all updates performed during the transaction into a log, and writes them 
%in-place only at transaction commit time, achieving data consistency for NVM without any modifications. 
%
%However, if the CPU caches are transient, transactional memory is not sufficient to guarantee persistence. We propose \sys, 
%a system based on a simple 
%micro-architectural extension to HTM to support persistence and synchronization simultaneously for transient caches. We use 
%TSX to approximate the performance on \sys on a real system and we  
%implement \sys using the SESC simulator~\cite{sesc}. To understand the behavior of an STM with transient caches, 
%we augment TinySTM with support for persistence, similarly to 
%Mnemosyne~\cite{mnemosyne}.

%We also consider an implementation based on undo logs and one based on redo logs. For multi-threaded applications, we protect the transactional 
%blocks with a global lock. Note, that this implementation still preserves the semantics of a transactional programming model, despite using locks. 
%In particular, nested transactions get flattened, and partial results do not become committed until the end of the transaction, unlike a programming model 
%based on locks, such as Atlas~\cite{atlas}.  

%We provide an extensive study of these (and other) crash consistency mechanisms for six representative applications and two NVM technologies (with persistent and transient 
%caches). 


%%summarize the result - insights from the eval 
%From this experience we learn these general trends:\\
%(1) In systems with transient caches, for both single and multi-threaded applications, crash consistent HTMs generally perform best.\\
%(2) In systems with persistent caches, for single-threaded applications, pure software based crash consistency mechanisms perform best. Moreover, \undo-logging approaches work better than \redo-logging approaches.\\
%(3) In systems with transient caches, for multi-threaded applications, crash consistent HTMs again
%are the best bet for application developers.
%



%Our empirical study results in the following conclusions:\\
%(1) The persistence domain significantly impacts the performance and programmability of transactional libraries. The cost of \cc and \cs for persistent caches is \ic{XX\% and YY} lower than for transient caches\ic{, respectively}. This suggests that NVM manufacturers and datacenter admins should consider increasing the persistence domain to the cache hierarchy, whenever possible (e.g. by augmenting the system with a battery).
%(2) \cc has a non-trivial overhead for both persistent \ic{(XX\%)} and transient caches\ic{(XX\%)}. However, techniques for ensuring multi-threaded \sync, such as STM and HTM, can help alleviate some of this overhead by 
%enabling applications to scale. Therefore, \cs generally has lower overhead when employing multiple threads \ic{(XX for persistent caches and XX for transient caches)} than \cc. 
%(3) While the \htm and \stm always outperform other methods for \cs for both persistent and transient caches, there is no clear winner between the two, as their behavior depends on the workload.
%(4) For \cc, the overhead of the \stm is too high when the application does not scale to more threads. However, the \htm still outperforms \undo/\redo logs for transient caches because it reduces the number of fences required. For persistent caches, where fences are not required, the \undo log outperforms all other methods. 
%\jg{We need numbers here and need to update so that most are on real NVM not DRAM anymore except simulator}.


%Limitations 
%Our study has the following limitation: NVM is not available yet, so we evaluate the different mechanisms using DRAM to approximate the behavior 
%of NVM and we simulation to implement the micro-architectural changes required to support \sys when caches are transient. \ic{What else?}


%This paper makes the following contributions:
%\begin{tightitemize}
%\item We provide an in-depth analysis of execution costs involved in different transactional techniques
%	using a real hardware platform.
%\item We propose HTM accelerated durable transaction system \sys and provide implementation
%	guidelines against the popular HTM realization found in Intel processors -- Intel TSX.
%\item We implement \sys in a software simulator environment that supports Intel TSX style 
%	HTMs. 
%% and present evaluation numbers and insights.
%Experimental results, gathered with 
%the popular STAMP benchmark~\cite{stamp}, 
%show that \sys outperforms storage 
%transactions by X\% and state-of-the-art persistent STMs by as much as Y\%.
%\end{tightitemize}
%


%summarize results from evaluation
%We implement \sys micro-architectural proposal in a simulator environment that already supporting
%faithful simulation of Intel TSX like HTMs. Next we evaluate \sys
%against STAMP benchmarks that is designed after number of enterprise
%application workloads. 
%The experimental results show that \sys outperforms storage 
%transactions by X\% and state-of-the-art persistent STMs by as much as Y\%.

%The paper is organized as follows. 
%First, we define \cs (\S\ref{pvs}) and discuss how to achieve it (\S\ref{sec:design}). Next, we explain our methodology (\S\ref{sec:methodology}), 
%and present an extensive evaluation of the 
%various implementations for \cc (\S\ref{sec:st-transient}) and for \cs (\S\ref{sec:mt-transient}).\ada{change labels to top section heading}











